Object-Region Video Transformers

Recently, video transformers have shown great success in video understanding, exceeding CNN performance; yet existing video transformer models do not explicitly model objects, although objects can be essential for recognizing actions. In this work, we present Object-Region Video Transformers (ORViT), an \emph{object-centric} approach that extends video transformer layers with a block that directly incorporates object representations. The key idea is to fuse object-centric representations starting from early layers and propagate them into the transformer-layers, thus affecting the spatio-temporal representations throughout the network. Our ORViT block consists of two object-level streams: appearance and dynamics. In the appearance stream, an "Object-Region Attention" module applies self-attention over the patches and \emph{object regions}. In this way, visual object regions interact with uniform patch tokens and enrich them with contextualized object information. We further model object dynamics via a separate "Object-Dynamics Module", which captures trajectory interactions, and show how to integrate the two streams. We evaluate our model on four tasks and five datasets: compositional and few-shot action recognition on SomethingElse, spatio-temporal action detection on AVA, and standard action recognition on Something-Something V2, Diving48 and Epic-Kitchen100. We show strong performance improvement across all tasks and datasets considered, demonstrating the value of a model that incorporates object representations into a transformer architecture. For code and pretrained models, visit the project page at \url{https://roeiherz.github.io/ORViT/}

==> Tables/abl_layer12.tex <==
\begin{tabularx}
{\linewidth}{@{}l c c c c}
    \toprule
    {Layers} & {Top-1} & {Top-5} & GFLOPs ($10^9$) & Param ($10^6$)\\ 
    \midrule
    Baseline & 60.2 & 85.8 & 370 & 109 \\ 
	1 & 68.8 & 90.4 & 381 & 122 \\ 
	1, 6 & 69.3 & 90.6 & 393 & 135 \\ 
	1, 6, 10 & \textbf{69.7} & \textbf{91.0} & 405 & 148 \\ 
    % \midrule
    % \bf CAMIN TimeSformer (Ours) & {\scriptsize IN-21K} & 32 & \bf 86.7 \\
\end{tabularx}

% param ($10^6$), GFLOPS ($10^9$)

% %%%% SSv2 Ablation - Layers
% \begin{tabularx}[t] 
% % 	\vspace{-15pt}
% 	\centering
% 	\small
% % 	\tablestyle{2pt}{1.05}
% % 	\resizebox{0.8\linewidth}{!}{
%     	\begin{tabular}{c|c|c|c|c|c}
%     		\multicolumn{1}{c|}{Depth}  &\multicolumn{1}{c|}{CAMIN Blocks} &   Top-1  & Top-5  & FLOPs ($10^9$)  & Params ($10^6$) \\

%     		\hline
%     		\multirow{4}{*}{12}  & - & 46.1 & 76.8 & 392 & 121 \\ 
%     		& 1 & 62.0 & 87.5 & 445 & 201 \\ 
%     		& 1, 6 & 63.1 & 88.3 & 498 & 281 \\ 
%     		& 1, 6, 10 & 63.5 & 88.7 & 551 & 361 \\

%     	\end{tabular}
% % 		}
% % 	}
% % 	\vspace{-1.4em}
% 	\label{tab:abl_layer12}
% \end{tabularx} 




==> Tables/abl_layers.tex <==
%%%% SSv2 Ablation - Layers
\begin{table}[t] 
% 	\vspace{-15pt}
	\centering
	\small
% 	\tablestyle{2pt}{1.05}
% 	\resizebox{0.8\linewidth}{!}{
    	\begin{tabular}{c|c|c|c|c|c}
    		\multicolumn{1}{c|}{Depth}  &\multicolumn{1}{c|}{CAMIN Blocks} &   Top-1  & Top-5  & FLOPs ($10^9$)  & Params ($10^6$) \\
    		
    		\hline
    		\multirow{4}{*}{4}  & - & 34.7 & 66.8 & 132 & 41 \\
    		& 1 & 58.8 & 85.3 & 185 & 121 \\
    		& 1, 2 & 57.9 & 84.6 & 238 & 201 \\ 
    		& 1, 2, 3 & 57.8 & 84.4 & 291 & 281 \\
    		
    		\hline
    		\multirow{5}{*}{6}  & - & 41.4 & 73.5 & 197 & 61 \\ 
    		& 1 & 60.8 & 86.6 & 250 & 141 \\ 
    		& 1, 2 & 60.1 & 86.2 & 303 & 221 \\ 
    		& 1, 3 & 59.6 & 86.1 & 303 & 221 \\
            & 1, 3, 4 & 59.4 & 85.8 & 356 & 301 \\
    		
    		\hline
    		\multirow{6}{*}{8}  & - & 44.9 & 77.0 & 262 & 81 \\ 
    		& 1 & 62.5 & 88.0 & 315 & 161 \\ 
    		& 1, 4 & 62.2 & 87.4 & 315 & 241 \\ 
    		& 1, 3, 5 & 61.5 & 86.8 & 421 & 321 \\
            & 1, 4, 6 & 61.5 & 86.9 & 368 & 241 \\
            & 1, 6 & 62.4 & 87.6 & 368 & 241 \\

    		\hline
    		\multirow{4}{*}{12}  & - & 46.1 & 76.8 & 392 & 121 \\ 
    		& 1 & 62.0 & 87.5 & 445 & 201 \\ 
    		& 1, 6 & 63.1 & 88.3 & 498 & 281 \\ 
    		& 1, 6, 10 & 63.5 & 88.7 & 551 & 361 \\
    % 		& 1, 3, 5 & 62.6 & 87.8 & 551 & 361 \\

    		\hline
    		\multirow{4}{*}{14}  & - & 45.6 & 77.1 & 457 & 141 \\ 
    		 & 1 & 62.2 & 87.5 & 510 & 221 \\ 
    		& 1, 7 & 63.0 & 88.0 & 563 & 301 \\ 
    		& 1, 7, 12 & 63.9 & 88.6 & 616 & 382 \\

    		\hline
    		\multirow{4}{*}{16}  & - & 45.2 & 76.9 & 522 & 161 \\ 
    		& 1 & 62.0 & 87.4 & 575 & 241 \\ 
    		& 1, 8 & 64.0 & 88.3 & 628 & 321 \\ 
    		& 1, 8, 14 & 63.5 & 88.4 & 681 & 402 \\

    	\end{tabular}
% 		}
% 	}
	\caption{\textbf{Layers ablation}. We ablate the layers to verify how many layers holds the most significant gain. In all experiments, we used an encoder with two layers and a kernel size of $3 \times 3$ in the convolution. Additionally, the experiments performed on the Compositional split in the SSv2 dataset. Magnitudes are Giga ($10^9$) for FLOPs and Mega ($10^6$) for Params. }
% 	\vspace{-1.4em}
	\label{tab:ablation:layer1}
\end{table} 

==> Tables/abl_layout.tex <==
\begin{tabularx}
{\linewidth}{@{}l c c r@{} r}
    \toprule
    {Model} & {Top-1} & {Top-5} \\ 
    \midrule
    Expand objects & 68.4 & 89.9 \\
    Tracklet Position Encoder (Ours) & \bf 69.7 & \bf 91.0 \\
    % \midrule
    % \bf CAMIN TimeSformer (Ours) & {\scriptsize IN-21K} & 32 & \bf 86.7 \\
    \bottomrule
\end{tabularx}


==> Tables/abl_location.tex <==
%%%% SSv2 Ablation - Location
\begin{table}[t] 
% 	\vspace{-15pt}
	\centering
	\small
% 	\tablestyle{2pt}{1.05}
% 	\resizebox{0.8\linewidth}{!}{
    	\begin{tabular}{c|c|c|c|c|c}
    		\multicolumn{1}{c|}{Depth}  & \multicolumn{1}{c|}{CAMIN Layers} &   Top-1  & Top-5  & \multicolumn{1}{c|}{FLOPs ($10^9$)} & \multicolumn{1}{c}{Params ($10^6$)} \\
    		
    		\hline
    		\multirow{4}{*}{4} & - & 34.7 & 66.8 & 132 & 41 \\
    		\cline{2-6}
    		& 1 & 59.0 & 85.2 & \multirow{3}{*}{185} & \multirow{3}{*}{121} \\ 
    		& 2 & 58.8 & 85.2 & & \\ 
    		& 3 & 33.6 & 75.8 & & \\
    		
    		\hline
    		\multirow{4}{*}{6}  & - & 41.4 & 73.5 & 197 & 61 \\
    		\cline{2-6}
    		& 1 & 60.8 & 86.6 & \multirow{3}{*}{250} & \multirow{3}{*}{141} \\ 
    		& 3 & 60.6 & 86.4 & & \\ 
    		& 4 & 59.6 & 86.1 & & \\

    		\hline
    		\multirow{4}{*}{8} & - & 44.9 & 77.0 & 262 & 81 \\
    		\cline{2-6}
    		& 1 & 62.5 & 88.0 & \multirow{3}{*}{315} & \multirow{3}{*}{161} \\ 
    		& 4 & 63.1 & 88.1 & & \\ 
    		& 6 & 62.6 & 87.8 & & \\

    		\hline
    		\multirow{4}{*}{12} & - & 46.1 & 76.8 & 392 & 121 \\
    		\cline{2-6}
    		& 1 & 62.1 & 87.5 & \multirow{3}{*}{445} & \multirow{3}{*}{201} \\ 
    		& 6 & 63.0 & 88.3 & & \\ 
    		& 10 & 62.1 & 87.7 & & \\
    	\end{tabular}
% 		}
% 	}
	\caption{\textbf{Location of Layers}. We ablate the layers to verify which layer holds the most significant gain. In all experiments, we used an encoder with two layers and a kernel size of $3 \times 3$ in the convolution. Additionally, the experiments performed on the Compositional split in the SSv2 dataset. Magnitudes are Giga ($10^9$) for FLOPs and Mega ($10^6$) for Params.}
% 	\vspace{-1.4em}
	\label{tab:ablation:layer2}
\end{table} 

==> Tables/abl_location12.tex <==
\begin{tabularx}
{\linewidth}{@{}c c c c c}
    \toprule
    {Layers} & {Top-1} & {Top-5} & GFLOPs ($10^9$) & Param ($10^6$)\\ 
    \midrule
	Baseline & 60.2 & 85.8 & 370 & 109 \\
	1 & 68.8 & 90.4 & 381 & 122 \\ 
	6 & 68.9 & 90.5 & 381 & 122 \\ 
	10 & 66.8 & 89.3 & 381 & 122 \\
\end{tabularx}


% %%%% SSv2 Ablation - Location
% \begin{table}[t] 
% % 	\vspace{-15pt}
% 	\centering
% 	\small
% % 	\tablestyle{2pt}{1.05}
% % 	\resizebox{0.8\linewidth}{!}{
%     	\begin{tabular}{c|c|c|c|c|c}
%     		\multicolumn{1}{c|}{Depth}  & \multicolumn{1}{c|}{CAMIN Layers} &   Top-1  & Top-5  & \multicolumn{1}{c|}{FLOPs ($10^9$)} & \multicolumn{1}{c}{Params ($10^6$)} \\
    		
%     		\hline
%     		\multirow{4}{*}{4} & - & 34.7 & 66.8 & 132 & 41 \\
%     		\cline{2-6}
%     		& 1 & 59.0 & 85.2 & \multirow{3}{*}{185} & \multirow{3}{*}{121} \\ 
%     		& 2 & 58.8 & 85.2 & & \\ 
%     		& 3 & 33.6 & 75.8 & & \\
    		
%     		\hline
%     		\multirow{4}{*}{6}  & - & 41.4 & 73.5 & 197 & 61 \\
%     		\cline{2-6}
%     		& 1 & 60.8 & 86.6 & \multirow{3}{*}{250} & \multirow{3}{*}{141} \\ 
%     		& 3 & 60.6 & 86.4 & & \\ 
%     		& 4 & 59.6 & 86.1 & & \\

%     		\hline
%     		\multirow{4}{*}{8} & - & 44.9 & 77.0 & 262 & 81 \\
%     		\cline{2-6}
%     		& 1 & 62.5 & 88.0 & \multirow{3}{*}{315} & \multirow{3}{*}{161} \\ 
%     		& 4 & 63.1 & 88.1 & & \\ 
%     		& 6 & 62.6 & 87.8 & & \\

%     		\hline
%     		\multirow{4}{*}{12} & - & 46.1 & 76.8 & 392 & 121 \\
%     		\cline{2-6}
%     		& 1 & 62.1 & 87.5 & \multirow{3}{*}{445} & \multirow{3}{*}{201} \\ 
%     		& 6 & 63.0 & 88.3 & & \\ 
%     		& 10 & 62.1 & 87.7 & & \\
%     	\end{tabular}
% % 		}
% % 	}
% 	\caption{\textbf{Location of Layers}. We ablate the layers to verify which layer holds the most significant gain. In all experiments, we used an encoder with two layers and a kernel size of $3 \times 3$ in the convolution. Additionally, the experiments performed on the Compositional split in the SSv2 dataset. Magnitudes are Giga ($10^9$) for FLOPs and Mega ($10^6$) for Params.}
% % 	\vspace{-1.4em}
% 	\label{tab:ablation:layer2}
% \end{table} 

==> Tables/ablations.tex <==
\begin{table*}[tb]
    \caption{\textbf{Albations.} We report pretrain, param ($10^6$), GFLOPS ($10^9$), and top-1 and top-5 action accuracy.}
    % \caption{\textbf{Albations.} We choose the recent \ocmodel~Mformer as our model and perform the ablations on the ``SomethingElse'' split. We report pretrain, param ($10^6$), GFLOPS ($10^9$), and top-1 and top-5 action accuracy.\amirg{a) Don't start explaining details of the ablation here (such as we chose mformer). b) Don't include flops. Probably top-5 is also not necessary. put in supp.}}
    \begin{subtable}[t]{.65\linewidth}
    % \tablestyle{3.5pt}{1.05}
    \scriptsize
        \centering
        \caption{\bf{Components}}
        % \renewcommand*{\arraystretch}{1.4}
        \label{tab:pitch}
		\input{Tables/abl_pitch}
	\end{subtable}
	% \hfill
	\begin{subtable}[t]{.32\linewidth}
    \tablestyle{6.0pt}{0.9}
    \scriptsize
        \centering
        \caption{\bf{\ocmodel~Modifications}}
        % \renewcommand*{\arraystretch}{3}
        \label{tab:abl_objsfusion}
		\input{Tables/abl_objsfusion}
	\end{subtable}
	\\
	\vspace{-0.8em}
    \begin{subtable}[t]{.3\linewidth}
    \tablestyle{4.5pt}{1.00}
    \scriptsize
        \centering
        \caption{\bf{Boxes}}
        % \renewcommand*{\arraystretch}{1.4}
        \label{tab:abl_boxes}
		\input{Tables/abl_boxes}
	\end{subtable}
	% \hfill
	\begin{subtable}[t]{.35\linewidth}
	\tablestyle{3.5pt}{1.2}
	\scriptsize
	    \centering
	    \caption{\bf{Streams}}
	   % \renewcommand*{\arraystretch}{1.19}
	    \label{tab:abl_streams}
	    \input{Tables/abl_streams}
	\end{subtable}
    % \quad
    % 	\hfill
    \begin{subtable}[t]{.33\linewidth}
    % \tablestyle{3.5pt}{1.05}
    \scriptsize
        \centering
        \caption{\bf{Object-Motion Module}}
        % \renewcommand*{\arraystretch}{3}
        \label{tab:abl_motion}
		\input{Tables/abl_motion}
	\end{subtable}

	\vspace{-0.8em}
    \label{tab:ablations}
    % \vspace{-0.5em}
\end{table*}









% All ablations!

% \begin{table*}[tb]
%     \caption{\textbf{Albations.} We choose the recent CAMIN-Mformer as our model and perform the ablations on the ``SomethingElse'' split. We report pretrain, param ($10^6$), GFLOPS ($10^9$), and top-1 and top-5 video action recognition accuracy.}
% 	\begin{subtable}[t]{.38\linewidth}
% % 	\tablestyle{2.5pt}{1.05}
% 	\scriptsize
% 	    \centering
% 	    \caption{\bf{Components}}
% 	   % \renewcommand*{\arraystretch}{1.19}
% 	    \label{tab:abl_streams}
% 	    \input{Tables/abl_streams}
% 	\end{subtable}
%     % \quad
%     % \hfill
%     \begin{subtable}[t]{.30\linewidth}
%     \scriptsize
%         \centering
%         \caption{\bf{Object-Region Attention}}
%         % \renewcommand*{\arraystretch}{3}
%         \label{tab:abl_appearance}
% 		\input{Tables/abl_appearance}
% 	\end{subtable}
%     % 	\hfill
%     % \quad
%     \begin{subtable}[t]{.3\linewidth}
%     \scriptsize
%         \centering
%         \caption{\bf{Boxes}}
%         % \renewcommand*{\arraystretch}{1.4}
%         \label{tab:abl_boxes}
% 		\input{Tables/abl_boxes}
% 	\end{subtable}
%     % \quad
% 	\\
% 	\vspace{-0.8em}

%     \begin{subtable}[t]{.48\linewidth}
%     \scriptsize
%         \centering
%         \caption{\bf{Layers Ablation}}
%         % \renewcommand*{\arraystretch}{1.4}
%         \label{tab:abl_layer12}
% 		\input{Tables/abl_layer12}
% 	\end{subtable}
%     % \hfill
%     \quad
%     \begin{subtable}[t]{.48\linewidth}
%     \scriptsize
%         \centering
%         \caption{\bf{Layers Location}}
%         % \renewcommand*{\arraystretch}{1.4}
%         \label{tab:abl_location12}
% 		\input{Tables/abl_location12}
% 	\end{subtable}
%     \\
%     \vspace{-0.8em}

%     \begin{subtable}[t]{.25\linewidth}
%     \scriptsize
%         \centering
%         \caption{\bf{Object-Motion Module}}
%         % \renewcommand*{\arraystretch}{3}
%         \label{tab:abl_motion}
% 		\input{Tables/abl_motion}
% 	\end{subtable}
% 	\hfill
%     % \quad
%     \begin{subtable}[t]{.33\linewidth}
%     \scriptsize
%         \centering
%         \caption{\bf{Object Fusion Methods}}
%         % \renewcommand*{\arraystretch}{3}
%         \label{tab:abl_objsfusion}
% 		\input{Tables/abl_objsfusion}
% 	\end{subtable}
%     \hfill
%     % \quad
%     \begin{subtable}[t]{.38\linewidth}
%     \scriptsize
%         \centering
%         \caption{\bf{Layout}}
%         % \renewcommand*{\arraystretch}{3}
%         \label{tab:abl_layout}
% 		\input{Tables/abl_layout}
% 	\end{subtable}
	
%     \label{tab:ablations}
%     \vspace{-1em}
% \end{table*}


==> Tables/sota_ava_smaller.tex <==
% \begin{tabularx}
% {\linewidth}{@{}l c c c c c}
% 	    \toprule
% 		{Model} & {Pretrain} &  {mAP}  & {Param} \\ 
% 		\midrule
% 		{SlowFast}, $4 \times 16$, R50 & {K400} & 21.9 & 33.7 \\ 
% 		SlowFast, $8 \times 8$, R101  & {K400} & 23.8  & 53.0 \\ 
% % 		\cline{1-1} \cline{3-5}
% 		{MViT}-B, $16 \times 4$   & {K400} & 25.5 & 36.4 \\ 
% 		\bf \ocmodel~MViT-B (Ours), $16 \times 4$   & {K400} & \bf 26.6 & - \\ 
% % 		{MViT}-B, $32 \times 3$    &  {K400} & 26.8 & 170 & 36.4 \\  
% % 		{MViT}-B, $64 \times 3$    &  {K400} & \textbf{27.3} & 455 & 36.4 \\  
		
% % 		\midrule
		
% % 		{SlowFast}, $8 \times 8$ R101+NL   & {K600}   &  27.1 & 147 & 59.2 \\ 
% % 		{SlowFast}, $16 \times 8$ R101+NL   &  {K600}  &  27.5 & 296 & 59.2 \\
% % 		X3D-XL &  {K600}  &  27.4 & 48.4 & 11.0 \\
% % % 		\cline{1-1} \cline{3-5}
% % 		{MViT}-B, $16 \times 4$   & {K600} & 26.1 & 70.5 & 36.3 \\ 
% % 		{MViT}-B, $32 \times 3$    &  {K600} & 27.5 & 170 & 36.4 \\ 
% % 		{MViT}-B-24, $32 \times 3$    & {K600} & \textbf{28.7} & 236& 52.9 \\  
% \end{tabularx}


\begin{wrapfigure}{r}{4.5cm}
    \vspace{-1.0em}
	\centering
	\tablestyle{1.0pt}{1.0}
	\scriptsize
	\begin{tabular}{l c c c c}
	    \toprule
		{Model} & {Pretrain} &  {mAP}  & {Param} \\ 
		\midrule
		{SlowFast}, $4 \times 16$, R50 & {K400} & 21.9 & 33.7 \\ 
		SlowFast, $8 \times 8$, R101  & {K400} & 23.8  & 53.0 \\ 
		\hline
		{MViT}-B, $16 \times 4$   & {K400} & 25.5 & 36.4 \\ 
		{MViT}-B, $32 \times 3$   & {K400} & 27.3 & 36.4 \\ 
		\hline
		\bf{\ocmodel~MViT-B, $16 \times 4$ (Ours)} & {K400} & \bf 26.6 & 49.8 \\
		\bf{\ocmodel~MViT-B, $32 \times 3$ (Ours)} & {K400} & \bf 28 & 49.8 \\
		\midrule
	\end{tabular}
	\vspace{-1.5em}
	\caption{\small Evaluation on AVA. %All methods use \textit{single center crop} inference.
	}
	\label{tab:sota_ava}
	\vspace{-2.0em}
\end{wrapfigure}

==> Tables/sota_diving48_smaller.tex <==
\begin{tabularx}
{\linewidth}{@{}l c r@{} r}
    \toprule
    {Model} & Frames & {Top-1} \\ 
    \midrule
    I3D & 8 & 48.3 \\
    TSM & 3 & 51.1 \\
    TSN & 3 & 52.5 \\
    % TRNms & ImageNet & 3 & 66.0\\
    GST-50 & 8 & 78.9 \\
    ST-S3D & 8 & 50.6 \\

    \midrule
    TimeSformer + STIN & 32 & 81.0 \\
    TimeSformer + STRG & 32 & 78.1 \\
    TimeSformer + STRG + STIN & 32 & 83.5 \\
    \midrule
    SlowFast, R101 & 16 & 77.6 \\
    TimeSformer  16 & 74.9 \\
    % TimeSformer & IN-21K & 32 & - \\
    TimeSformer-HR & 16 & 78.0 \\
    TimeSformer-L & 96 & 81.0 \\
    TQN & ALL & 81.8  \\

    \midrule
    \bf \ocmodel~TimeSformer (Ours) & 32 & \bf 88.0\gcol{$+$6.2} \\
    \bottomrule
\end{tabularx}


==> Tables/sota_epic_kitchens_smaller.tex <==
\begin{tabularx}
    {\linewidth}{@{}l c c c}
    \toprule
    {Method} & {A} & {V} & {N}  \\ 
    \midrule
    TSN &  33.2 & 60.2 & 46.0 \\ 
    TRN & 35.3 & 65.9 & 45.4 \\ 
    TBN & 36.7 & 66.0 & 47.2 \\
    TSM & 38.3 & 67.9 & 49.0 \\
    SlowFast & 38.5 & 65.6 & 50.0 \\
    
    \midrule
    Mformer-HR + STIN & 44.2 & 67.0 & 57.9 \\
    Mformer-HR + STRG & - & - & - \\
    Mformer-HR + STRG + STIN & 44.1 & 66.9 & 57.8 \\
    \midrule
    TimeSformer & 32.9 & 55.8 & 50.1 \\
    ViViT-L & 44.0 & 66.4 & 56.8 \\
    Mformer & 43.1 & 66.7 & 56.5 \\
    Mformer-L & 44.1 & 67.1 & 57.6 \\
    Mformer-HR & 44.5 & 67.0 & \bf 58.5 \\
    
    \midrule
    \bf \ocmodel~Mformer-HR & \bf \scriptsize 45.5\gcol{$+$1.0} & \bf \scriptsize 68.3\gcol{$+$1.3} & \scriptsize 58.2\rcol{$-$.3} \\
    \bottomrule
\end{tabularx}


==> Tables/sota_ssv2.tex <==
\renewcommand*{\thefootnote}{\fnsymbol{footnote}}
\begin{tabularx}
{0.9\linewidth}{@{}l c c c c r@{} c}
% {0.85\linewidth}{@{}l c c c c r@{} r}
    \toprule
    {Model} & Boxes & Pretrain & {Top-1} & {Top-5} & {GFLOPs$\times$views} ($10^9$) & {~~~~Param} ($10^6$)\\ 
    \midrule
    % SlowFast, R50 & \xmark & K400 & 61.7 & 87.0 & 65.7$\times$3$\times$1 & 34.1 \\
    SlowFast, R101 & \xmark & K400 & 63.1 & 87.6 & 106$\times$3$\times$1 & 53.3 \\
    % TSM & \xmark & K400 & 63.4 & 88.5 & 62.4$\times$3$\times$2 & 42.9\\
    % STM & \xmark & IN-1K & 64.2 & 89.8 & 66.5$\times$3$\times$10 & - \\
    % MSNet & \xmark & IN-1K & 64.7 & 89.4 & 67$\times$1$\times$1 & 24.6 \\
    % TEA & \xmark & IN-1K & 65.1 & - & 70$\times$3$\times$10 & - \\
    % bLVNet & \xmark & IN-1K & 65.2 & 90.3 & 128.6$\times$3$\times$10 & - \\
    % \midrule
    % VidTr-L & \xmark & {\scriptsize IN+K400} &  60.2 & - & 351$\times$3$\times$10 & - \\ 
    TimeSformer-L & \xmark & IN & 62.5 & - & 1703$\times$3$\times$1 & 121.4 \\
    ViViT-L & \xmark & {\scriptsize IN+K400}  & 65.4 & 89.8 & 3992$\times$4$\times$3 & -\\
    % MViT-B, 32 & \xmark & K400  &  67.1 &  90.8 & 170$\times$3$\times$1 & 36.6 \\
    % MViT-B, 64 & \xmark & K400  &  67.7 &  90.9 & 455$\times$3$\times$1 & 36.6 \\
    % MViT-B, 32 & \xmark & K600  &  67.8 &  91.3 & 170$\times$3$\times$1 & 36.6 \\
    MViT-B, 64 & \xmark & K600  &  68.7 &  91.5 & 236$\times$3$\times$1 & 53.2 \\

    \midrule
    
    \Mformer & \xmark & {\scriptsize IN+K400} & 66.5 & 90.1 &$369.5\times3\times1$ & 109 \\
    % \Mformer & \xmark & {\scriptsize IN+K600} & 66.5 & 89.8 &$369.5\times3\times1$ & 109\\
    % \Mformer-HR & \xmark & {\scriptsize IN+K400}  & 67.1 & 90.6 & $958.8\times3\times1$ & -\\

    % \Mformer + STIN & GT & {\scriptsize IN+K400} &  66.9 &  89.4 & $369.5\times3 \times1$ & 111 \\
    % \Mformer + STRG & GT & {\scriptsize IN+K400} &  69.1 &  90.9 & $375\times3 \times1$ & 117 \\

    \Mformer-L & \xmark & {\scriptsize IN+K400} & 68.1 & 91.2 &$1185.1\times3 \times1$ & 109 \\

    \Mformer + STRG + STIN  & GT & {\scriptsize IN+K400} &  69.2 &  90.9 & $375\times3 \times1$ & 119 \\
    
    \midrule
    
    \bf \ocmodel~\Mformer  (Ours) & Detected & {\scriptsize IN+K400}  & \textbf{67.9}\gcol{$+$1.4} & 90.5\gcol{$+$0.4} & $405\times3 \times1$ & 148\\
    \bf \ocmodel~\Mformer  (Ours) & GT & {\scriptsize IN+K400}  & \textbf{73.8}\gcol{$+$7.3} & \textbf{93.6}\gcol{$+$3.5} & $405\times3 \times1$ & 148\\
    % \bf \ocmodel~\Mformer (Ours) & GT & {\scriptsize IN+K400}  & \textbf{71.4}\gcol{$+$4.9} & \textbf{91.8}\gcol{$+$1.7} & $405\times3 \times1$ & 148\\
    \bf \ocmodel~\Mformer-L  (Ours) & Detected & {\scriptsize IN+K400}  & \bf 69.5\gcol{$+$1.4} & \bf 91.5\gcol{$+$0.3} & $ 1259\times3 \times1$ & 148.2 \\
    \bf \ocmodel~\Mformer-L (Ours) & GT & {\scriptsize IN+K400}  & \textbf{74.9}\gcol{$+$6.7} & \textbf{94.2}\gcol{$+$3.0} & $ 1259\times3 
    % \bf \ocmodel~\Mformer-L \footnotemark[\value{footnote}] (Ours) & GT & {\scriptsize IN+K400}  & \textbf{73.5}\gcol{$+$5.4} & \textbf{93.3}\gcol{$+$2.1} & $ 1259\times3
    \times1$ & 148.2\\

    \bottomrule
\end{tabularx}

% \begin{tabularx}
% {0.65\linewidth}{@{}l c c c r@{} r}
%     \toprule
%     {Model} & Pretrain & {Top-1} & {Top-5} & {GFLOPs$\times$views} & {~~Param} \\ 
%     \midrule
%     SlowFast, R50 & K400 & 61.7 & 87.0 & 65.7$\times$3$\times$1 & 34.1 \\
%     SlowFast, R101 & K400 & 63.1 & 87.6 & 106$\times$3$\times$1 & 53.3 \\
%     TSM & K400 & 63.4 & 88.5 & 62.4$\times$3$\times$2 & 42.9\\
%     STM & IN-1K & 64.2 & 89.8 & 66.5$\times$3$\times$10 & - \\
%     MSNet & IN-1K & 64.7 & 89.4 & 67$\times$1$\times$1 & 24.6 \\
%     TEA & IN-1K & 65.1 & - & 70$\times$3$\times$10 & - \\
%     bLVNet & IN-1K & 65.2 & 90.3 & 128.6$\times$3$\times$10 & - \\
%     \midrule
%     VidTr-L & {\scriptsize IN+K400} &  60.2 & - & 351$\times$3$\times$10 & - \\ 
%     TimeSformer-L & IN & 62.5 & - & 1703$\times$3$\times$1 & 121.4 \\
%     ViViT-L & {\scriptsize IN+K400}  & 65.4 & 89.8 & 3992$\times$4$\times$3 & -\\
%     MViT-B, 32 & K400  &  67.1 &  90.8 & 170$\times$3$\times$1 & 36.6 \\
%     MViT-B, 64 & K400  &  67.7 &  90.9 & 455$\times$3$\times$1 & 36.6 \\
%     MViT-B, 32 & K600  &  67.8 &  91.3 & 170$\times$3$\times$1 & 36.6 \\
%     \Mformer & {\scriptsize IN+K400} & 66.5 & 90.1 &$369.5\times3\times1$ & -\\
%     \Mformer-HR & {\scriptsize IN+K400}  & 67.1 & 90.6 & $958.8\times3\times1$ & -\\
%     \Mformer-L & {\scriptsize IN+K400} & 68.1 & 91.2 &$1185.1\times3 \times1$ & - \\
%     MViT-B, 64 & K600  &  68.7 &  91.5 & 236$\times$3$\times$1 & 53.2 \\
    
%     \midrule
%     \bf CAMIN \Mformer (Ours) & {\scriptsize IN+K400}  & \bf 71.4 & \bf 91.8 & $958.8\times3\times1$ & -\\
%     \bf CAMIN \Mformer-L (Ours) & {\scriptsize IN+K400}  & \bf 73.5 & \bf 93.3 & $958.8\times3\times1$ & -\\
%     \bottomrule
% \end{tabularx}


% \begin{tabularx}
% {\linewidth}{@{}l c c c r@{}}
%     \toprule
%     {Model} & Pretrain & {Top-1} & {Top-5} & GFLOPs $\times$ views \\ 
%     \midrule
%     SlowFast~\citep{slowfast2019} & K-400 & 61.7 & - & 65.7$\times$3$\times$1\\
%     TSM~\citep{Lin_2019_ICCV} & K-400 & 63.4 & 88.5 & 62.4$\times$3$\times$2 \\
%     STM~\citep{stm} & IN-1K & 64.2 & 89.8 & 66.5$\times$3$\times$10 \\
%     MSNet~\citep{kwon2020motionsqueeze} & IN-1K & 64.7 & 89.4 & 67$\times$1$\times$1 \\
%     TEA~\citep{li2020tea} & IN-1K & 65.1 & - & 70$\times$3$\times$10 \\
%     bLVNet~\citep{blvnet2019neurips} & IN-1K & 65.2 & 90.3 & 128.6$\times$3$\times$10 \\
%     \midrule
%     VidTr-L~\citep{li2021vidtr} & {\scriptsize IN+K-400} &  60.2 & - & 351$\times$3$\times$10 \\ 
%     Tformer-L~\citep{bertasius2021spacetime} & IN & 62.5 & - & 1703$\times$3$\times$1 \\
%     ViViT-L~\citep{arnab2021vivit} & {\scriptsize IN+K-400}  & 65.4 & 89.8 & 3992$\times$4$\times$3 \\
%     MViT-B~\citep{fan2021multiscale} & K-400  &  67.1 &  90.8 & 170$\times$3$\times$1 \\
%     \Mformer~\citep{arnab2021vivit} & {\scriptsize IN+K-400} & 66.5 & 90.1 &$369.5\times3\times1$ \\
%     \Mformer-L~\citep{arnab2021vivit} & {\scriptsize IN+K-400} & \bf 68.1 & \bf 91.2 &$1185.1\times3 \times1$ \\
%     \Mformer-HR~\citep{arnab2021vivit} & {\scriptsize IN+K-400}  & 67.1 & 90.6 & $958.8\times3\times1$ \\
    
%     \midrule
    
%     \bottomrule
% \end{tabularx}


        % Model & Top-1 & Top-5  \\ 
        % \midrule
        % TRN~\citep{zhou2017temporalrelation} & 48.8 & 77.6  \\
        % TRN-DATNN~\citep{xiao2019reasoning}  & 51.6 &  80.3  \\
        % SF~\citep{slowfast2019} & 61.7 & - \\
        % TimeSformer~\citep{bertasius2021spacetime} & 62.6 & - \\
        % TSM~\citep{Lin_2019_ICCV} & 63.4 & 89.8 \\
        % % STIN~\citep{materzynska2019something} & 48.4 & 78.7\\
        % % I3D & 55.5 & 81.4 \\
        % % I3D + STIN & 60.2 & 84.4 \\
        % STM~\citep{stm} & 64.2 & - \\
        % TEA~\citep{tea_2020_CVPR} & 65.1 & - \\
        % blVNET~\citep{blvnet2019neurips} & 65.2 & \textbf{90.3} \\
        % ViViT~\citep{arnab2021vivit} & 65.4 & 89.8 \\
        % \Mformer~\citep{arnab2021vivit} & 65.4 & 89.8 \\
        
        

==> Tables/sota_ssv2_comp_fewshot_orig.tex <==
\begin{table}[t!]
%   \vspace{-1.5em}
  \scriptsize
  \caption{\textbf{Compositional and Few-Shot Action Recognition} on the ``SomethingElse'' dataset. All results are reported using ground-truth box annotations.}
%   \vspace{-0.3em}
  \tablestyle{2.5pt}{1.00}
   \centering
    \begin{tabular}{l c cc cc cc cc}
            \toprule
            % \multirow{2}{*}{{Model}} & {RGB} & {Boxes} & {Top-1} & {Top-5} \\ 
            
            \multirow{2}{*}{{Model}} & \multicolumn{2}{c}{Modality} & \multicolumn{2}{c}{Compositional} & \multicolumn{2}{c}{Base} & \multicolumn{2}{c}{Few-Shot} \\ 
            
             & {RGB} & {Boxes} & {Top-1} & {Top-5} & {Top-1} & {Top-5} & {5-Shot} & {10-Shot}  \\
            
            % \cmidrule(l{0pt}r{0pt}){2-3} 
            \midrule
            {I3D~\cite{carreira2017quo}} & \cmark & \xmark & 42.8 & 71.3 & 73.6 & 92.2 & 21.8 & 26.7 \\
            {SF~\cite{slowfast2019}} & \cmark & \xmark & 45.2 & 73.4 & 76.1 & 93.4 & 22.4 & 29.2 \\
            {TimeSformer~\cite{gberta_2021_ICML}} & \cmark & \xmark & 44.2 & 76.8 & 79.5 & 95.6 & 24.6 & 33.8 \\
            {Mformer~\cite{patrick2021keeping}} & \cmark & \xmark &  60.2 & 85.8 & 82.8 & 96.2 & 28.9 & 33.8 \\

            \midrule
            % {STIN (OIE + NL)~\cite{materzynska2019something}} & \cmark & \cmark &  42.2 & 71.5 \\
            % {SF + STIN (OIE + NL)~\cite{materzynska2019something}} & \cmark & \cmark &  52.3 & 78.5 \\
            
            {STRG (\textbackslash{w}~SF)~\cite{Wang_videogcnECCV2018}} & \cmark & \cmark &  52.3 & 78.3 & 75.4 & 92.7 & 24.8 & 29.9 \\
            % {STIN~\cite{materzynska2019something}} & \cmark & \cmark &  51.4 & 79.3 & 70.2 & 91.4 & 17.2 & 25.4 \\
            {STIN} (\textbackslash{w}~SF)~\cite{materzynska2019something} & \cmark & \cmark &  54.6 & 79.4 & 77.4 & 95.0 & 23.0 & 33.4 \\
            % {STIN} (ensemble)~\cite{materzynska2019something} & \cmark & \cmark &  58.1 & 83.2 & 76.1 & 92.7 & 27.3 & 32.6 \\
            % {Mformer+STRG} & \cmark & \cmark &  61.8 & 86.3 & - & - & - & - \\
            % {Mformer+STIN} & \cmark & \cmark &  61.8 & 85.9 & - & - & - & - \\
            {Mformer+STRG+STIN} & \cmark & \cmark &  62.3 & 86.0 & 83.7 & 96.8 & 29.8 & 36.5 \\
            % \textsc{MGAF~\cite{}}($32$ Frames) & \cmark & \cmark &  68.0 & 88.7 & - & - & - & -\\
            \midrule
            
            \bf {\ocmodel~Mformer (ours)} & \cmark & \cmark & \bf {{69.7}} & \bf {{91.0}} & \bf 87.1 & \bf 97.6 & \bf 33.3 & \bf 40.2 \\
            \bottomrule
   \end{tabular}%
    \label{tab:comp_fewshot}
    % \vspace{-.2cm}
\end{table}
% \vspace{-1em}

==> Tables/sote_ssv2_comp.tex <==



\begin{table}[ht]
  \scriptsize
  \centering
    \begin{tabular}{c c cc cc cc}
            \toprule
            % \multirow{2}{*}{{Model}} & {RGB} & {Boxes} & {Top-1} & {Top-5} \\ 
            
            \multirow{2}{*}{{Model}} & \multicolumn{2}{c}{Modality} & \multicolumn{2}{c}{SSv2} & \multicolumn{2}{c}{IKEA Assembly} \\ 
            
             & {RGB} & {Boxes} & {Top-1} & {Top-5} & {Top-1} & {Top-5} \\
            
            % \cmidrule(l{0pt}r{0pt}){2-3} 
            \midrule
            \textsc{I3D~\citep{carreira2017quo}} & \cmark & \xmark & 42.8 & 71.3 \\
            \textsc{SF~\citep{slowfast2019}} & \cmark & \xmark & 45.2 & 73.4 \\
            \textsc{TimeSformer~\citep{gberta_2021_ICML}} & \cmark & \xmark & 44.2 & 76.8 & 72.4 & 96.3 \\
            \textsc{MFormer~\citep{patrick2021keeping}} & \cmark & \xmark &  60.2 & 85.8 & 75.1 & 95.2 \\

            \midrule
            % \textsc{STIN (OIE + NL)~\citep{materzynska2019something}} & \cmark & \cmark &  42.2 & 71.5 \\
            % \textsc{SF + STIN (OIE + NL)~\citep{materzynska2019something}} & \cmark & \cmark &  52.3 & 78.5 \\
            
            \textsc{STIN~\citep{materzynska2019something}} & \cmark & \cmark &  51.4 & 79.3 \\
            \textsc{STRG~\citep{Wang_videogcnECCV2018}} & \cmark & \cmark &  52.3 & 78.3 \\
            \textsc{STIN} (\textbackslash{w}~SF)~\citep{materzynska2019something} & \cmark & \cmark &  54.6 & 79.4 \\
            \textsc{STIN} (ensemble)~\citep{materzynska2019something} & \cmark & \cmark &  58.1 & 83.2 & - & - \\
            % \textsc{MGAF~\citep{}}($32$ Frames) & \cmark & \cmark &  68.0 & 88.7 & - & -\\

            \midrule
            
            \bf \textsc{CAMIN Mformer (ours)} & \cmark & \cmark & \bf {{69.8}} & \bf {{90.6}} \\
            \bottomrule
  \end{tabular}%
  \caption{\textbf{Compositional Action Recognition.}}
    \label{tab:compar}
\end{table}


% \begin{table}[ht]
%   \centering
%     \begin{tabular}{c c cc cc cc}
%             \toprule
%             \multirow{2}{*}{{Model}} & \\
%             & \multicolumn{3}{c}{Ground-truth Boxes} & \multicolumn{3}{c}{\textsc{Tracker}~\cite{materzynska2019something} Boxes} \\
 
%             & Boxes & {Top-1} & {Top-5} & Boxes & {Top-1} & {Top-5} \\ 
%             % \cmidrule(l{0pt}r{0pt}){2-3} 
%             \midrule
%             \textsc{I3D~\cite{carreira2017quo}} & \xmark & 42.8 & 71.3 & \xmark & 42.8 & 71.3\\
%             \textsc{SF~\cite{slowfast2019}} & \xmark & 45.2 & 73.4 & \xmark & 45.2 & 73.4 \\
%             \textsc{TimeSformer~\cite{bertasius2021spacetime}} & \xmark & 44.2 & 76.8 & \xmark & 44.2 & 76.8 \\
            
%             \textsc{STIN (OIE + NL)~\cite{materzynska2019something}} & \cmark &  42.2 & 71.5 & \cmark & 30.0 & 64.8 \\
%             \textsc{SF + STIN (OIE + NL)~\cite{materzynska2019something}} & \cmark &  52.3 & 78.5 & \cmark & 47.7 & 74.0 \\
%             % \textsc{SF + STIN (OIE + NL)~\cite{materzynska2019something}} & \cmark &  50.2 & 77.4 & \textsc{Tracker}~\cite{materzynska2019something} & 47.7 & 74.0 \\
%             \midrule
%             \midrule

            
%             \textsc{1 stream (combined)} & \cmark  & {53.0} & {79.9} & \cmark & {46.1} & {72.3} \\
%             \textsc{1 stream (motion)} & \cmark & 55.0 & 81.9 & \cmark & 49.2 & 75.3 \\
%             \textsc{2 streams, fully decoupled} & \cmark  & {{54.6}} & {{80.7}} & \cmark & {49.2} & {75.5} \\
%             \textsc{2 streams, partially decoupled} & \cmark  & \textbf{{{56.7}}} & \textbf{{{82.1}}} & \cmark & \textbf{{50.9}} & \textbf{{77.6}} \\
            
%             % \midrule

%             % \textsc{SF + APPIM} (1 stream, combined) & \cmark & 53.0 & 79.9 & \cmark & 46.1 & 72.3 \\

%             % \textsc{OTIN (SF + APPIM + MOTIM)} & \cmark  & \textbf{{56.7}} & \textbf{{82.1}} & \cmark & {50.1} & {77.6} \\
            
%             \bottomrule
%   \end{tabular}%
%   \caption{\textbf{Compositional Action Recognition on SSv2.} The GT boxes were annotated by humans, while the detected boxes have been produced by different models. For STIN~\cite{materzynska2019something}, we used their proposed tracker for the detected boxes, while for our method, we used our the Tube Attention module (\textsc{TUBE-ATT}) in an end-to-end manner. We note that \textbf{our OTIN model$^{*}$ with the \textsc{TUBE-ATT}, requires boxes only for training and not at inference time}, unlike the previous methods (e.g., STIN~\cite{materzynska2019something}, etc.) or when using the GT boxes.}
%     \label{tab:compar}
% \end{table}

==> Tables/sote_ssv2_fewshot.tex <==
\begin{table}[ht]
  \scriptsize
   \centering
    \begin{tabular}{c c cc cc cc}
            \toprule
            \multirow{2}{*}{{Model}} & 
            \multicolumn{1}{c}{{\textit{Boxes}}} & \multicolumn{2}{c}{{\textit{Base}}} & \multicolumn{2}{c}{{\textit{Few-Shot}}}\\ 
            & & {Top-1} & {Top-5} & {5-shot} & {10-shot}\\ 
            \midrule
            \textsc{I3D~\citep{carreira2017quo}} & \xmark & 73.6 & 92.2 & 21.8 & 26.7\\
            \textsc{SF~\citep{slowfast2019}} & \xmark & 76.1 & 93.4 & 22.4 & 29.2 \\
            % \textsc{TimeSformer~\citep{gberta_2021_ICML}} & \xmark & 79.5 & 95.6 & 24.4 & 33.7 \\
            % \textsc{STIN}~\citep{materzynska2019something} & \textsc{GT} & 70.2 & 91.4 & 27.7 & 33.5\\
            \textsc{STIN}~\citep{materzynska2019something} & \cmark & 68.1 & 89.6 & 17.2 & 25.4 \\
            \textsc{SF + STIN~\citep{materzynska2019something}} & \cmark & 77.4 & 95.0 & 23.0 & 33.4 \\
            % \textsc{SF + STIN~\citep{materzynska2019something}} & \textsc{Tracker}~\citep{materzynska2019something} & {70.3} & {90.8} & {17.4} & {20.7} \\

            \midrule
            
            \bf \textsc{CAMIN} & \cmark & \textbf{83.2} & \textbf{96.5} & \textbf{33.6} & \textbf{42.4} \\
            
            \bottomrule
   \end{tabular}%
   \caption{\textbf{Few-Shot Compositional Action Recognition} on SSv2. For the detected tubes, please refer to the supp~\secref{tab:fewshot_full}.}
    \label{tab:fewshot}
\end{table}



% \begin{table}[ht]
%   \scriptsize
%   \centering
%     \begin{tabular}{c c cc cc cc}
%             \toprule
%             \multirow{2}{*}{{Model}} & 
%             \multicolumn{1}{c}{{\textit{Boxes}}} & \multicolumn{2}{c}{{\textit{Base}}} & \multicolumn{2}{c}{{\textit{Few-Shot}}}\\ 
%             & & {Top-1} & {Top-5} & {5-shot} & {10-shot}\\ 
%             \midrule
%             \textsc{I3D~\citep{carreira2017quo}} & \xmark & 73.6 & 92.2 & 21.8 & 26.7\\
%             \textsc{SF~\citep{slowfast2019}} & \xmark & 76.1 & 93.4 & 22.4 & 29.2 \\
%             % \textsc{TimeSformer~\citep{bertasius2021spacetime}} & \xmark & 79.5 & 95.6 & 24.4 & 33.7 \\
%             % \textsc{STIN}~\citep{materzynska2019something} & \textsc{GT} & 70.2 & 91.4 & 27.7 & 33.5\\
%             \textsc{STIN}~\citep{materzynska2019something} & \textsc{GT} & 68.1 & 89.6 & 17.2 & 25.4 \\
%             \textsc{SF + STIN~\citep{materzynska2019something}} & \textsc{GT} & 77.4 & 95.0 & 23.0 & 33.4 \\
%             % \textsc{SF + STIN~\citep{materzynska2019something}} & \textsc{Tracker}~\citep{materzynska2019something} & {70.3} & {90.8} & {17.4} & {20.7} \\
%             \textsc{SF + STIN~\citep{materzynska2019something}} & \textsc{Tracker}~\citep{materzynska2019something} & {70.3} & {90.8} & {19.4} & {27.7} \\
            
%             \midrule
            
%             \textsc{1 stream (combined)} & \textsc{GT} & {80.9} & {95.8} & {27.3} & {32.5} \\
%             \textsc{1 stream (motion)} & \textsc{GT} & {83.2} & {96.4} & {33.3} & {42.4} \\
%             \textsc{2 streams, fully decoupled} & \textsc{GT} & \textbf{{83.2}} & {96.5} & \textbf{{33.6}} & \textbf{{42.4}} \\
%             \textsc{2 streams, partially decoupled} & \textsc{GT} & {83.1} & {96.5} & {32.5} & {41.0} \\

%             \midrule
%             \textsc{DITIN} & \textsc{GT} & \textbf{83.2} & \textbf{96.5} & \textbf{33.6} & \textbf{42.4} \\
%             \textsc{DITIN} & \textsc{Tracker}~\citep{materzynska2019something} & {77.8} & {94.0} & {23.5} & {29.3} \\
%             % \textsc{DITIN} & \textsc{E2E} & {77.4} & {93.6} & {20.5} & {29.3} \\

%             \bottomrule
%   \end{tabular}%
%   \caption{\textbf{Few Shot Compositional Action Recognition} on SSv2. For the detected tubes, please refer to the supp~\secref{tab:fewshot_full}.}
%     \label{tab:fewshot}
% \end{table}

==> supp_clean.tex <==
% % \usepackage{hyperref}
% \newpage
\clearpage
% \setcounter{section}{0} %% Start counting from the beginning

% \title{Supplementary Material for ``Object-Region Video Transformers''}

% \title{Supplementary Material for ``TubeIN''}

% \section{Appendix}
In this supplementary file, we provide additional information about our model, implementation details, experimental results, and qualitative examples. Specifically,~\Secref{supp:impl} provides additional implementation details,~\Secref{supp:model} provides additional model details, ~\Secref{supp:ablations} provides additional ablations of our approach,~\Secref{supp:exper} provides more experiment results, and we show qualitative visualizations to demonstrate our approach in~\Secref{supp:qual}.

% Finally, in Section~\ref{supp:experiments} we provide additional baseline implementation details and more evidence regarding AG2Vid performance.


\section{Additional Implementation Details}
\label{supp:impl}
We add {\ocmodel} to the existing transformer models \Mformer, MViT and TimesFormer. These are all implemented based on the SlowFast~\cite{slowfast2019} library (available at \url{https://github.com/facebookresearch/SlowFast}) and we base our code on that library.  Next, we elaborate on how we extract the object regions, and for each dataset, we add additional implementation details.


\subsection{Detector and Tracker} 
\label{supp:impl:det_tracker}
\minisection{Detector} In all action recognition datasets we used Faster R-CNN detector~\cite{nips2015fastercnn,maskrcnn2017iccv} with ResNet-50 backbone~\cite{resnet1} and Feature Pyramid Network (FPN)~\cite{Lin2017FeaturePN} that is pre-trained on the MS~COCO~\cite{Lin2014MSCOCO} dataset. We used the Detectron2 implementation. In SSv2, the detector is finetuned using the bounding boxes annotation supplied in the Something Else dataset, during the finetune the class categories are \textit{hand} and \textit{object} involved in action. For AVA, we used the supplied detection boxes for the spatio-temporal action detection task that were first obtained by Faster-RCNN pre-trained over MS~COCO and then fine-tuned on AVA as in~\cite{lfb2019}. We set the number of objects in our model to 4 in SSv2 and EK100, 6 in AVA, and 10 in Diving48. If fewer objects are presented, we set the object coordinates with a zero vector.

\minisection{Tracker} Once we have the detector results, we apply multi-object tracking to find correspondence between the objects in different frames. We use SORT~\cite{Bewley2016_sort}: a simple tracker implemented based on Kalman Filter~\cite{Klman1960ANA} and the Hungarian matching algorithm (KM). At each step, the Kalman Filter predicts plausible instances in the current frame based on previous tracks. Next, the predictions are matched with single-frame detections by the Hungarian matching algorithm. It is important to note that the tracker does not require any training and does not use any additional data. If an object does not appear in one of the frames, we set the coordinates in these frames to zeros.

% \minisection{Tracker} Once we have the detector results, we apply multi-object tracking to find correspondence between the objects in different frames. The multi-object tracker is a simple tracker implemented based on Kalman Filter~\cite{Klman1960ANA} and the Hungarian matching algorithm (KM)~\cite{Kuhn1955TheHM} following~\cite{Bewley2016_sort}. At each step, the Kalman Filter predicts plausible instances in the current frame based on previous tracks. Next, the predictions are matched with single-frame detections by the Hungarian matching algorithm.


\subsection{Something-Something v2}
\label{supp:impl:ssv2}
\minisection{Dataset.} SSv2~\cite{goyal2017something} contains 174 action categories of common human-object interactions. We follow the official splits from~\cite{materzynska2019something} to train and test our model for action recognition, compositional action recognition, and few-shot.

\minisection{Optimization details} For the standard SSv2~\cite{materzynska2019something} dataset, we trained $16$ frames with sample rate $4$ and batch-size $48$ on $8$ RTX 3090 GPUs. We train our network for 35 epochs with Adam optimizer with a momentum of $0.9$ and Gamma $0.1$. Following~\cite{patrick2021keeping}, we use $lr = 5e-5$ with $\times10$ decay steps at epochs $0, 20, 30$. Additionally, we used Automatic Mixed Precision, which is implemented by PyTorch. We initialize from a Kinetics-400 pre-trained model~\cite{kay2017kinetics}. For the \textit{\ocmodel~\Mformer-L} model, we fine-tuned from the SSv2 pre-trained model provided by~\cite{patrick2021keeping} and train with $32$ frames. The optimization policy is similar to the above, except we used a different learning rate: $1e-5$ for the pre-trained parameters, and $1e-4$ for the {\ocmodel} parameters. 

For the compositional action recognition task, we trained on the SomethingElse splits~\cite{materzynska2019something}. We train with a batch size of $32$ and a learning rate of $3e-5$.

\minisection{Regularization details} We use weight decay of $0.05$, a dropout of $0.5$ before the final classification, dropout of $0.3$ after the \ocmodel~block, and DropConnect with rate $0.2$.

\minisection{Training details} We use a standard crop size of $224$, and we jitter the scales from $256$ to $320$. Additionally, we use RandAugment with maximum magnitude $20$ for each frame separately.

\minisection{Inference details} We take 3 spatial crops per single clip to form predictions over a single video in testing as done in ~\cite{patrick2021keeping}.


% we adopt a half-period cosine schedule of learning decaying and use a linear warm-up startegy . 




% Following~\cite{patrick2021keeping}, we adopt a half-period cosine schedule of learning decaying and use a linear warm-up startegy

% For Action Genome~\cite{ji2019action}, we trained $16$ frames with base size $8$. We train our network for 35 epochs  using synchronous SGD, and initialization from a Kinetics-400~\cite{kay2017kinetics} pretrained model. For optimization we use SGD with $lr = 0.01$ with $10 \times$ learning-rate decay, momentum of $0.9$ and weight decay of $1e^{-6}$.

\subsection{EpicKitchens100}
\label{supp:impl:ek100}

\minisection{Dataset} EK100~\cite{Damen2020RESCALING100EPIC} contains 700 egocentric videos of daily kitchen activities. This dataset includes 300 noun and 97 verb classes, and we report verb, noun, and action top-1 accuracy, while the highest-scoring of the verb and noun pairs constitutes the action label.

\minisection{Optimization details} We trained over videos of $16$ frames with sample rate $4$ and batch-size $16$ on $8$ Quadro RTX 8000 GPUs. We train our network for 35 epochs with Adam optimizer with a momentum of $0.9$ and Gamma $0.1$. Following~\cite{patrick2021keeping}, we use $lr = 5e-5$ with $\times10$ decay steps at epochs $0, 30, 40$. Additionally, we used Automatic Mixed Precision, which is implemented by PyTorch. We initialize from a Kinetics-400 pre-trained model~\cite{kay2017kinetics}.

\minisection{Training details} We use crop size of $336$ for the \textit{\ocmodel~\Mformer-HR}. We jitter the scales from $384$ to $480$. Additionally, we use RandAugment with maximum magnitude $20$.

\minisection{Inference details} We take 3 spatial crops with 10 different clips sampled randomly to aggregate predictions over a single video in testing.




\subsection{Diving48}
\label{supp:impl:diving48}

\minisection{Dataset} Diving48~\cite{Li_2018_Diving48} contains 16K training and 3K testing videos spanning 48 fine-grained diving categories of diving activities. For all of these datasets, we use standard classification accuracy as our main performance metric. 


\minisection{Optimization details} We trained over videos of $32$ frames with sample rate $8$ and batch-size $8$ on $8$ Quadro RTX 8000 GPUs. We train our network for 35 epochs with Adam optimizer with a momentum of $0.9$ and Gamma $0.1$. We use $lr = 3.75e-5$ with $\times10$ decay steps at epochs $0, 20, 30$. Additionally, we used Automatic Mixed Precision, which is implemented by PyTorch. We initialize from a Kinetics-400 pre-trained model~\cite{kay2017kinetics}.

\minisection{Training details} We use a standard crop size of $224$ for the standard model and jitter the scales from $256$ to $320$. Additionally, we use RandomFlip augmentation. Finally, we sampled the $T$ frames from the start and end diving annotation time, followed by~\cite{zhang2021tqn}. 

\minisection{Inference details} We take 3 spatial crops per single clip to form predictions over a single video in testing same as in~\cite{gberta_2021_ICML}.

\minisection{Object-Dynamics Module} As we show in~\tabref{supp:tab:abl_motion}, we compared different self-attention mechanisms, and the standard self-attention usually performed better. However, we observe a slight improvement when we perform a trajectory self-attention~\cite{patrick2021keeping} instead of the standard self-attention. 


\subsection{AVA}
\label{supp:impl:ava}

\minisection{Architecture} SlowFast~\cite{slowfast2019} and MViT~\cite{mvit2021} are using a detection architecture with a RoI Align head on top of the spatio-temporal features. We followed their implementation to allow a direct comparison. Next we elaborate on the RoI Align head proposed in SlowFast~\cite{slowfast2019}. First, we extract the feature maps from our \ocmodel~MViT model by using the RoIAlign layer. Next, we take the 2D proposal at a frame into a 3D RoI by replicating it along the temporal axis, followed by a temporal global average pooling. Then, we max-pooled the RoI features and fed them to an MLP classifier for prediction. %Finally, we found that the ``Object-Dynamics Module'' did not contribute to the final results (the results are the same with or without it), and thus we decided to drop it for faster training.

\minisection{Optimization details} To allow a direct comparison, we used the same configuration as in MViT~\cite{mvit2021}. We trained $16$ frames with sample rate $4$, depth of $16$ layers and batch-size $32$ on $8$ RTX 3090 GPUs. We train our network for 30 epochs with an SGD optimizer. We use $lr = 0.03$ with a weight decay of $1e-8$ and a half-period cosine schedule of learning rate decaying. We use mixed precision and fine-tune from an MViT-B, $16\times4$ pre-trained model. 


% \minisection{Regularization details} Same as others.


% \subsection{Regularization details}
% We use weight decay of $0.05$, a dropout of $0.5$ before the final classification, dropout of $0.3$ after the CAMIN block, and dropconnect with rate $0.2$.

\minisection{Training details} We use a standard crop size of $224$ and we jitter the scales from $256$ to $320$. We use the same ground-truth boxes and proposals that overlap with ground-truth boxes by $IoU > 0.9$ as in~\cite{slowfast2019}.

\minisection{Inference details} We perform inference on a single clip with $16$ frames. For each sample, the evaluation frame is centered in frame $8$. We use a crop size of $224$ in test time. We take 1 spatial crop with 10 different clips sampled randomly to aggregate predictions over a single video in testing.

% \subsection{Something-Else}
% \label{supp:impl:ssv2}
% \minisection{Dataset.} SomethingElse~\cite{materzynska2019something}
% Several video datasets define an action via a combination of a verb (action) and noun (object). In such cases, it is more challenging to recognize combinations that were not seen during training. This ``compositional'' setting was explored in the ``SomethingElse'' dataset \cite{materzynska2019something}, where verb-noun combinations in the test data do not occur in the training data. The split contains 174 classes with 54,919/54,876 videos for training/validation. This setting is of particular relevance for object-centric models like {\ocmodel}, which can potentially better handle compositional actions. 

% \minisection{Optimization details} For the standard SSv2~\cite{materzynska2019something} dataset, we trained $16$ frames with sample rate $4$ and batch-size $48$ on $8$ RTX 3090 GPUs. We train our network for 35 epochs with Adam optimizer~\cite{kingma2014adam} with a momentum of $0.9$ and Gamma $0.1$. Following~\cite{patrick2021keeping}, we use $lr = 5e-5$ with $\times10$ decay steps at epochs $0, 20, 30$. Additionally, we used Automatic Mixed Precision, which is implemented by PyTorch. We initialize from a Kinetics-400 pre-trained model~\cite{kay2017kinetics}. For the \textit{\ocmodel~\Mformer-L} model, we fine-tuned from the SSv2 pre-trained model provided by~\cite{patrick2021keeping} and train with $32$ frames. The optimization policy is similar to the above, except we used a different learning rate: $1e-5$ for the pre-trained parameters, and $1e-4$ for the {\ocmodel} parameters. 

% For the compositional action recognition task, we trained on the SomethingElse splits~\cite{materzynska2019something}. We train with a batch size of $32$ and a learning rate of $3e-5$.

% \minisection{Regularization details} We use weight decay of $0.05$, a dropout of $0.5$ before the final classification, dropout of $0.3$ after the \ocmodel~block, and DropConnect with rate $0.2$.

% \minisection{Training details} We use a standard crop size of $224$, and we jitter the scales from $256$ to $320$. Additionally, we use RandAugment with maximum magnitude $20$ for each frame separately.

% \minisection{Inference details} We take 3 spatial crops per single clip to form predictions over a single video in testing as done in ~\cite{patrick2021keeping}.

\subsection{Few Shot Compositional Action Recognition}
\label{supp:impl:fewshot}

We also evaluate on the few-shot compositional action recognition task in~\cite{materzynska2019something}. For this setting, we have 88 \textit{base} action categories and 86 \textit{novel} action categories. We train on the base categories (113K/12K for training/validation) and finetune on few-shot samples from the novel categories (for 5-shot, 430/50K for training/validation; for 10-shot, 860/44K for training/validation).




\section{Additional Model details}
\label{supp:model}


\subsection{Object-Region Attention}
\label{supp:model:ocmodel}


As explained in~\secref{sec:model:ocmodel}, there are two inputs to the {\ocmodel} block. The first is the output of the preceding transformer block, represented as a set of spatio-temporal tokens  $X\in \reals^{THW \times d}$. The second input is a set of bounding boxes for objects across time, provided by an off-the-shelf object detector or available directly in the dataset. These bounding boxes are denoted by $B\in \reals^{T O\times 4}$.

\minisection{Object-Region Attention} Given the patch token features $X$ and the boxes $B$, we use RoIAlign~\cite{maskrcnn2017iccv} layer, which uses the patch tokens $X$ and box coordinates $B$ to obtain object region crops. This is followed by max-pooling and an MLP. To these features we add a learnable object-time position encoding $\mathcal{P} \in \reals^{TO \times d}$ to encode the positional object information. We also use a coordinate embedding by applying an MLP on the boxes coordinates, resulting in $\mathcal{L} \in \reals^d$:
\begin{equation}
    \mathcal{L} := \text{MLP}(B)
\label{eq:supp:location_embd}
\end{equation}

where $B \in \reals^{T \times O \times d}$ is the boxes coordinates. This leads to an improved object features:
\begin{equation}
     \mathcal{O} := \text{MLP}(\text{MaxPool}(\text{RoIAlign}(X,B))) + \mathcal{L} + \mathcal{P}
\label{eq:supp:objects}
\end{equation}

where the token features are $X \in \reals^{THW \times d}$. We pass these features into the self-attention layers as explained in the ``Object-Region attention'' subsection.

\ignore{
\minisection{Object-Dynamics Module} In the main paper, we explained how we use the coordinate embeddings and object-time position embedding to generate $\widetilde{B}$ (See Object-Dynamics Module in~\secref{sec:model}). Additionally, we use hand/object indicator identity for SSv2. We have two types of possible indicator annotations for each box: (i) \textit{Hand indicator} (hand in action), and (ii) \textit{Object indicator} (objects involved in the action with the hand). We use this information by placing the hand box in the first object index in the O dimension. We note the identity could be used by our prediction or the provided ground truth if it exists (whether collected with human annotations or by pseudo detections from detectors). For AVA and Diving48, we do not assume any indicator between the boxes (they are all objects).
}


% Additionally, we use the identity embedding to specify a learnable $d$-dimensional embedding representing the identities of objects and agents. We define three types of embedding: (i) \textit{Agent embedding} (person or hand in action); (ii) \textit{Object embedding} (objects involved in the action with the hand/person), and (iii) \textit{Background embedding} (null boxes that irrelevant to the action). We note that we could use the identity embedding by using our prediction or the provided ground truth if it exists (whether collected with human annotations or by pseudo detections from detectors). For SSv2, we use the ``hand'' as the agent embedding, while for EK100, we use ``left-hand'' and ``right-hand''. For AVA and Diving48, we use the object and background embeddings without agent.


% \subsection{Light-weighted Object-Dynamic Module}
% \label{supp:model:lightweight}

% We show in our ablations that the Object-Dynamic Module improves by $2.3\%$ the top1 accuracy with an additional 37M parameters. Here, we present a light-weighted version that removes all additional parameters without losing significant accuracy. The main idea is to share the position and location embeddings (as explained above) between the two modules in the \ocmodel~block: the ``Object-Region Attention'' and the ``Object-Dynamic Module''. \roei{Add details + results table}

% It shows that our main approach is the main reason for the observed improvements and not necessarily more parameters.







\section{Additional Ablations}
\label{supp:ablations}

\input{Tables/ablations_supp}

We perform an ablation study of each of the components in~\tabref{supp:tab:ablations} to show the effectiveness of the different components of our model. All ablations are on the SomethingElse dataset and use \Mformer as the baseline architecture for {\ocmodel} unless stated otherwise.


\minisection{Contribution of Appearance and motion Streams} In~\tabref{supp:tab:abl_streams}, we show the ``Object-Region Attention'' is an important factor for the improvement, responsible for a $7.2\%$ gain from the baseline without significant parameters addition (2M parameters compared to the baseline). This highlights our contribution that object interactions are indeed crucial for video transformers. Additionally, adding trajectory information with coordinates in the ``Object-Dynamics Module'' improved by another $2.3\%$.


\minisection{\ocmodel~Blocks} In~\tabref{supp:tab:abl_layer12_all}, we show which layers are most important for adding the \ocmodel~block. The experiments show that adding this information at the network's beginning, middle, and the end is the most effective (layer 2, 7, 11). We also note that, surprisingly, adding {\ocmodel} at the second layer has the most significant contribution ($8.6\%$ improvements).


\minisection{Different self attention in ``Object-Region Attention''} In~\tabref{supp:tab:abl_appearance}, we compared different self-attention mechanisms: joint space-time, divided space-time, and trajectory attention to the \textit{\Mformer} baseline, which uses trajectory attention in all layers. We observed that trajectory attention is slightly better.
% more suited to our block since the pairwise information between the objects and patch tokens propagates slightly better.
However, it can be seen that our object region approach is not sensitive to these choices, indicating that the generic approach is the main reason for the observed improvements.


% In~\tabref{supp:tab:abl_appearance}, we compared different self-attention mechanisms: joint space-time, divided space-time, and trajectory attention to the \textit{\Mformer} baseline, which uses trajectory attention in all layers. We observed that trajectory attention is more suited to our work since the pairwise information between the objects and patches propagates slightly better. However, it can be seen our object approach is improving regardless of which attention we choose.



\minisection{Processing trajectory information} In~\tabref{supp:tab:abl_motion}, we compared our self-attention (see ``Object-Dynamics Module'' in~\Secref{sec:model:ocmodel}) with other standard baseline models: GCN and trajectory self-attention~\cite{patrick2021keeping}. For the GCN, we use a standard implementation with 2 hidden layers, while for the trajectory attention, we treat the $O$ objects as the spatial dimension. Our model improves the GCN baseline by $2.0\%$, and the difference between the self-attention layers is significant ($0.3\%$ difference).


% For the RNN we used the standard pytorch implenetation with 3 layers applied over the coordinate embeddings.

% Additionally, we validated that our ``Box Position Encoder'' is more efficient for generating a layout from a $TO \times d$ tracklets embeddings compared to a standard tensor expansion (namely, expand the each object representation over the whole spatial dimension) by improving the top-1 video classification results on the SomethingElse dataset from $68.4\%$ to $69.7\%$. 


\minisection{Components on Diving48} Following our ablations in~\tabref{tab:pitch}, we also validate our approach on the Diving48 dataset in~\tabref{supp:tab:pitch_diving}. We used the TimeSformer trained on videos of $32$ frames as a baseline for a fair comparison. It can be seen that a single layer version of the model already results in considerable improvement ($85.4\%$) and that it is important to apply it in the earlier layers of transformers than at the end ($86.8\%$ compared to $85.4\%$). Additionally, the ``Object-Dynamics Module'' improves performance to $87.5\%$. Finally, multiple applications of the layer further improve performance to $88.0\%$. 



\minisection{Replacing {\ocmodel} with Trajectory Attention} We observe that Joint and Divided self attention layers~\cite{gberta_2021_ICML,arnab2021vivit} have similar results to the Trajectory Attention~\cite{patrick2021keeping}, as seen in~\tabref{supp:tab:abl_appearance}. However, we would like to demonstrate that Trajectory Attention is not the main reason for the improvement. Thus, we replace our {\ocmodel} with a standard Trajectory Attention on the Diving48 and AVA datasets. The top1 accuracy on Diving48 are improved by $4.5\%$ (from $80.0$ to $84.5$) with trajectory attention, while using our \textit{\ocmodel+TimeSformer} achieves $88.0$ ($3.5\%$ improvements on top of that). The MAP on AVA are the same as the baseline with trajectory attention ($25.5$), while using our \textit{\ocmodel+MViT-B} achieves $26.6$ ($1.1$ improvements on top of the baseline). We note that our \Mformer is the baseline on EK100, SSv2, and SomethingElse, and therefore the trajectory attention is already part of the model, and hence this demonstration is not needed.

\minisection{Box Position Encoder} Our ``Box Position Encoder'' transforms from a tensor of size $TO$ to  size $THW$. Our implementation of this transformation uses box information so that each object is mapped to the ``correct'' region in space. A simpler approach would have been to expand the shape of $TO$ to $THW$ without using boxes. We refer to the latter as a standard tensor expansion. Comparing the two methods, we find out that our approach obtains $69.7$ compared to $68.4$, showing that our box-based encoding performs better.


% \minisection{Components} In~\tabref{supp:tab:abl_streams}, we show the ``Object-Region Attention'' is an important factor for the improvement, responsible for a $7.2\%$ gain from the baseline without significant parameters addition (2M parameters compared to the baseline). The only difference compared to the baseline is the MLP addition after the RoIAlign layer. This highlights our contribution that object interactions are indeed crucial for video transformers. Additionally, adding motion information with coordinates in ``Object-Dynamic Module'' improved by another $2.3\%$.

% \minisection{Boxes} To validate the importance of object regions, we experimented different versions of boxes in~\tabref{tab:abl_boxes}: (i) \textit{Full boxes} - coordinates of the entire image $([0,0,1,1])$. (ii) \textit{Null boxes} - coordinates are initialized to zeros, and we removed the RoIAlign layer. (iii) \textit{Grid boxes} - divided the images into four fixed grids. (iv) \textit{Random boxes} - we select randomized coordinates for the image. We can learn that random boxes or fixed grids are not adding any new information, unlike object regions. Additionally, using null boxes shows that adding additional params is not the main reason for the improvements. Moreover, the full boxes ablation shows that adding the complete image information does not help the model better focus on the significant object region. Specifically, it shows that these object regions serve as a strong inductive bias for the model. Finally, we performed shuffling on the boxes and observed a degradation to $68.2$ top-1 accuracy, which means that the transformer can track by himself without the tracking information.

% \minisection{Object Fusion Methods} In~\tabref{supp:tab:abl_objsfusion}, we show three different baseline modifications that support our argument that adding object-centric information into transformers is not trivial. (i) \textit{Object Tokens} - We extract the object features from the RoIAlign layer and add them as tokens for the queries. It is interesting to see the performance is lower when using fixed object representations in the beginning, unlike our approach in which in every \ocmodel~layer, we obtain new object features by the RoIAlign. (ii) \textit{MF + RoIAlign} - We present a baseline that uses global and visual object representations. First, we used the RoIAlign layer on top of the global features to extract the object feature from the \Mformer. Then, we concatenated the global features with the object features and classified the action. Since we did not use object interactions between the ROIs, it might suggest that object interactions are an essential key factor in our model. (iii) \textit{MF + Coord} - We present a baseline that uses coordinates and global representations. We used the global features from the \Mformer model concatenated with motion embeddings. To calculate the motion embeddings, we use a standard self-attention over the coordinates.

% \minisection{\ocmodel~Blocks} In~\tabref{supp:tab:abl_layer12_all}, we show which layers are most important for adding the \ocmodel~block. The experiments show that adding this information at the network's beginning, middle, and the end is the most effective (layer 1, 6, 10). For more layer ablations, please refer to the supplementary. We also note, that surprisingly adding at the first layer is already good enough and has the most significant contribution ($8.6\%$ improvements).

% \minisection{Object-Region Attention} In~\tabref{supp:tab:abl_appearance}, we compared different self-attention mechanisms: joint space-time, divided space-time, and trajectory attention. We observed that trajectory attention is more suited to our work since the pairwise information between the objects and patches propagates slightly better. However, it can be seen our object approach is improving regardless of which attention we choose. 

% \minisection{Object-Dynamic Module} In~\tabref{supp:tab:abl_motion}, we compared our self-attention module with other standard baseline models: GCN and RNN. Our model improves on top of them. Additionally, we validated that our ``Tracklet Position Encoder'' is more efficient for generating a layout from a $TO \times d$ tracklets embeddings compared to a standard tensor expansion by improving the top-1 video classification results on SmthElse from $68.4\%$ to $69.7\%$. 







\input{Tables/lightweight_supp}


\section{Additional Experiments}
\label{supp:exper}

Here we present additional results of the standard action recognition task. Additionally, we show a lightweight version of the ``Object-Dynamics Module'' that significantly reduces the model parameters without losing significant performance.




\subsection{Light-weight Object-Dynamics Module}
\label{supp:exper:lightweight}



In~\tabref{supp:tab:abl_streams}, we show that the ``Object-Dynamics Module'' improves by $2.3\%$ the top-1 accuracy with an additional 39M parameters (148M Vs. 109M). We would like to demonstrate that our main approach is the main reason for the observed improvements and not necessarily the addition of more parameters. Here, we present a light-weight version of the module that reduces the embedding dimensions without losing significant accuracy. See~\tabref{tab:lightweight}. 

As mentioned in the main paper (see~\Secref{sec:model}), we use $\widetilde{B}$ for the coordinate embeddings and object-time position embedding in the ``Object-Dynamics Module''. We validate how the dimension size of $\widetilde{B}$ is responsible for the action accuracy. We observe that reducing the dimension of $\widetilde{B}$ from $768$ to $256$ has little impact on the action accuracy in SSv2 ($73.8\%$ Vs. $73.7\%$ for ground-truth boxes and $67.9\%$ Vs. $67.3\%$ for detected boxes) and SomethingElse ($68.7\%$ Vs. $67.9\%$), although having only 114M model parameters (only addition of 5M parameters to the \Mformer baseline that has 109M).

Indeed this indicates that our main approach is the main reason for the observed improvements and not necessarily more parameters.




\subsection{Results}
\label{supp:exper:results}

We next report in~\tabref{supp:table:ar} the full results table for the standard action recognition task, including extra models, which were not included in the main paper.

\begin{table*}[tb!]
    \caption{\textbf{Comparison to the state-of-the-art on video action recognition.} We report pretrain, param ($10^6$), GFLOPS ($10^9$) and top-1 ($\%$) and top-5 ($\%$) video action recognition accuracy on SSv2. We also report when our model uses ground-truth (GT) and detected boxes. On Epic-Kitchens100 (EK100), we report top-1 ($\%$) action (A), verb (V), and noun (N) accuracy. On Diving48 we report pretrain, number of frames and top-1 ($\%$) video action recognition accuracy. For EK100 and Diving48 we used only detected boxes since ground-truth does not exist.}
    
    \begin{subtable}[t]{.99\linewidth}
% 	\scriptsize
	\tablestyle{3.5pt}{1.05}
	    \centering
	    \setlength{\tabcolsep}{3pt}
	    \caption{\bf{Something--Something V2}}
		\input{Tables/sota_ssv2_supp}
		\label{supp:tab:sota_ssv2}
	\end{subtable}
	\\
    
    \begin{subtable}[t]{.45\linewidth}
    \tablestyle{4.5pt}{1.05}
    % \scriptsize
        \centering
        \caption{\bf{Diving48}}
        \label{supp:tab:sota_diving48}
		\input{Tables/sota_diving48_supp}
	\end{subtable}
	\hfill
	\begin{subtable}[t]{.55\linewidth}
	\tablestyle{4.5pt}{1.05}
% 	\scriptsize
	    \centering
	    \caption{\bf{Epic-Kitchens100}}
	    \label{supp:tab:sota_ek100}
	    \input{Tables/sota_epic_kitchens_supp}
	\end{subtable}
    \label{supp:table:ar}
    % \vspace{-10em}
\end{table*}




% \section{Datasets}
% \label{supp:exper:datasets}
% We use multiple datasets for both compositional and standard action recognition and spatio-temporal action detection. Next, we elaborate on them.

% \minisection{SSv2}~\cite{goyal2017something} contains 174 action categories of common human-object interactions. We follow the official splits from~\cite{materzynska2019something} to train and test our model for action recognition, compositional action recognition, and few-shot.

% \minisection{EK100}~\cite{Damen2020RESCALING100EPIC} contains 700 egocentric videos of daily kitchen activities. This dataset includes XXX noun and XX verb classes, and we report verb, noun, and action top1 accuracy, while the highest-scoring of the verb and noun pairs constitutes the action label.

% \minisection{Diving48}~\cite{Li_2018_Diving48} contains 16K training and 3K testing videos spanning 48 fine-grained diving categories of diving activities. For all of these datasets, we use standard classification accuracy as our main performance metric. 

% \minisection{AVA}~\cite{AVA2018} is a dataset with for human actions detection contains 211k training and 57k validation videos. We follow the standard protocol reporting Mean Average Precision (mAP) on 60 classes on AVA-V2.2.

% \textbf{(2) EK100~\cite{Damen2020RESCALING100EPIC}} contains 700 egocentric videos of daily kitchen activities. This dataset contains XXX noun and XX verb classes. This recent collection enables us to better test the compositionalities of nouns and verbs since it provide more complete annotations of fine-grained actions (+128\% more noun and verb categories with their times), unlike other datasets.



% \textbf{(2) Action Genome~\cite{ji2019action}} is built upon the Charades~\cite{sigurdsson2016hollywood} dataset, which captures human activities in daily life. We follow the official split to train and test our model. It has 35 object classes and 25 relation classes. For more details, please refer to the supplementary~\secref{supp:exper:datasets}.




%   \textbf{(3) Charades~\cite{sigurdsson2016hollywood}} We follow the official split (8K training and 1.8K validation videos) to train and test our model. The average video duration is around 30 seconds with 157 multiple action classes and we report our results by the metric of mean Average Precision (mAP). This dataset is challenging because of the high degree of overlap in the action instances. % Videos in the dataset contain an average of 6 action instances per video with an average of 79\% of overlapping instances in a video

\section{Qualitative Visualizations}
\label{supp:qual}
To provide insight into the inner representation of {\ocmodel} we provide further visualization next. 
See~\figgref{fig:vis1} and~\figgref{fig:vis2}. In~\figgref{fig:vis1}, we visualize the attention map of the CLS token on all spatial tokens. It can be seen that object-regions indeed affect these spatial maps. For example, ``Tearing something into two pieces'' (top left corner) demonstrates that \textit{\ocmodel+\Mformer} successfully separates the two pieces of the paper, while the \textit{\Mformer} baseline does not. Next, in~\figgref{fig:vis2} we visualize the attention allocated to each of the object keys. It can be seen that the object keys in \textit{\ocmodel} indeed affect their corresponding spatial tokens. 


\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/Visualizations_Figure1.pdf}
    % \vspace{-0.3cm}
    \caption{\textbf{Attention Maps} comparison between the \textit{\ocmodel+\Mformer} and the \textit{\Mformer} on videos from the SSv2 dataset. The visualization shows the attention maps corresponding to the CLS query.}
    \label{fig:vis1}
\end{figure*}


\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/Visualizations_Figure2.pdf}
    % \vspace{-0.3cm}
    \caption{\textbf{Object contribution to the patch tokens.} For each object token, we plot the attention weight given by the patch tokens, normalized over the patch tokens.}
    \label{fig:vis2}
\end{figure*}

